Selfless Sequential Learning

Sequential learning, also called lifelong learning, studies the problem of learning tasks in a sequence with access restricted to only the data of the current task. In this paper we look at a scenario with fixed model capacity, and postulate that the learning process should not be selfish, i.e. it should account for future tasks to be added and thus leave enough capacity for them. To achieve Selfless Sequential Learning we study different regularization strategies and activation functions. We find that imposing sparsity at the level of the representation (i.e.~neuron activations) is more beneficial for sequential learning than encouraging parameter sparsity. In particular, we propose a novel regularizer, that encourages representation sparsity by means of neural inhibition. It results in few active neurons which in turn leaves more free neurons to be utilized by upcoming tasks. As neural inhibition over an entire layer can be too drastic, especially for complex tasks requiring strong representations, our regularizer only inhibits other neurons in a local neighbourhood, inspired by lateral inhibition processes in the brain. We combine our novel regularizer, with state-of-the-art lifelong learning methods that penalize changes to important previously learned parts of the network. We show that our new regularizer leads to increased sparsity which translates in consistent performance improvement %over alternative regularizers we studied on diverse datasets.

==> approach_old.tex <==
\section{Selfless Sequential Learning (\textbf{SNI})}
\label{sec:method}


As explained earlier, the main problem in sequential learning is catastrophic forgetting of previous tasks as a result of learning new tasks. In order to prevent catastrophic forgetting, importance weight based methods proceed by introducing  an importance weight $\Omega_{k}$ for each parameter $\theta_{k}$ in the network. %Elastic weight consolidation~\cite{kirkpatrick2016overcoming} computes the Fisher information matrix, while~\cite{zenke2017improved} ... Rotate your network, Remanian walk and Memory Aware Synapses.
While these methods differ in how to estimate the important parameters  as discussed in the related work section, all of them 
penalize the changes on the important parameters  when learning a new task $T_n$  using $L_2$ penalty as follows:
\begin{equation} 
T_n:\quad \min_{\theta} \frac{1}{M} \sum_{m=1}^{M}  l(y_m,f(x_m,\theta))+ \lambda_{\Omega}\sum_{k} \Omega_{k}(\theta_{k}-\theta^*_{k})^2
\end{equation}
where $\theta^*_{k}$ are the optimal parameters that are learned so far, i.e. before the current task.  $x_m$ is the input and $y_m$ the desired output  of the network. $\lambda_{\Omega}$ is a trade-off parameter between the new  task objective and the changes on the important parameters.\\
Our goal is to impose a regularization mechanism that encourages the learning procedure of a given task in a sequence to learn sparse and decorrelated representation. This in turn  minimizes the interference with the previous and future tasks and as well as utilizes fewest possible number of neurons.
To promote sparsity in the representation, we can identify, in the literature, the use of  $L_1$ norm on the activations since minimizing the  $L_0$ norm is an NP hard problem. It has been  suggested by~\cite{pmlr-v15-glorot11a} to be combined with the rectifier activation function (ReLU) to control the unbounded activations and to increase the sparsity. However,  $L_1$ norm imposes an equal penalty on all the active neurons leading to small activation magnitude across the network.
\marcus{add one or more citation where L1 is used in LLL}\rahaf{we are the first to propose this in LLL, however, there is a new ICML paper that uses L1 penalty on some masks on the activations in a similar spirit but in a different regime, not sure how to integrate this. }\\
On the other hand,  learning decorrelated representation has been explored before  under the goal of reducing overfitting. This is usually done by minimizing the Forbenious norm of the covariance matrix corrected by the diagonal as in \cite{cogswell2015reducing} or \cite{xiong2016regularizing}. Such a penalty results in a decorrelated representation but with activations that are mostly close to a non zero mean value.
Merging the two objectives of sparse and decorrelated representation can be achieved by the following objective:

\begin{equation}
\label{eq:appraoch:regularizer:simple}
R(H_l)=\frac{1}{M}  \sum_{i,j}\sum_m  h_i^mh_j^m  ,  \quad i\neq j
\end{equation}
where we consider a hidden layer $l$ with the activations $H_l=\{h^m_{i}\}$ given an input example $x_m$ where $i \in {1,..,N}$ with $N$ the  number of neurons in the hidden layer.
 This formula differs from minimizing the Forbenious norm of the covariance matrix  in two simple yet important aspects:\\
 1- In the case of a ReLU activation function, used in most of the modern architectures, a neuron is active  if its output is larger than zero and zero otherwise. By assuming a close to zero mean of the neurons activations $ \mu_i \simeq 0 \, \forall i \in {1,..,N}$, it minimizes the neurons correlation between any two active neuorns.\\
%t
% Thus, we consider having a mean close to zero  to discourSage the neurons' activations from frequently having nonzero values.  in 
%\begin{equation}
2- By evaluating the derivative of the presented regularizer w.r.t. activation, we get:
\begin{equation}
\frac {\partial R(H_l)}{\partial h_i^m}=\frac{1}{M}   \sum_{j\neq i} h_j^m
\end{equation}
each active neuron receives a penalty from every other active neuron that corresponds to that other neuron's activation magnitude. In other  words, if a neuron fires, with a high activation value, for a given example, it will suppress firing other neurons for that same example. Hence, this would result in a decorrelated sparse representation.\\ 
%, hence the name of our regularizer Sparse coding through Neural Inhibition, {\tt SNI} for short. 
The loss imposed by this objective will only be zero when there is exactly one active neuron per example. This seems to be too harsh for complex examples that need a richer representation. Thus, we suggest to relax the objective by imposing a spatial weighting to the correlation penalty. 
In other words, an active neuron penalizes mostly its close neighbours and this effect vanishes for further neurons. 
\marcus{is there something like a "wrap around"? i.e. does i=1 suppress j=N, otherwise there will be a arbitrary border effect, i.e. not all neurons are equal.}
Instead of uniformly penalizing all the neurons correlation, we weight the correlation penalty between each two neurons by the probability density of a random variable $X \sim N(0,\sigma^2)$
\marcus{clarify how $P(x_{ij})$ and $P(0)$ are defined}
\begin{equation}
\label{eq:appraoch:regularizer:first}
%R_{\textrm{SNI}}(H_l)=\frac{1}{M} \sum_{i,j} \frac{P(x_{ij})}{P(0)}\sum_m  h_i^mh_j^m  ,  \quad i\neq j
R_{\textrm{SLNI}}(H_l)=\frac{P(x_{ij})}{P(0)} R(H_l) = \frac{1}{M} \sum_{i,j} \frac{P(x_{ij})}{P(0)}\sum_m  h_i^mh_j^m  ,  \quad i\neq j
\end{equation}
\marcus{I tried to make the connection to \ref{eq:appraoch:regularizer:simple}}
\marcus{As I said it would be good to ablate to \ref{eq:appraoch:regularizer:simple} in the experiments}
at ${x_{ij}=i-j}$ for two neurons locations $n_i,n_j$ proportional to the probability density at zero\rahaf{the division by zero is to ease the tuning of the hyper parameter and to get a value close to 1 for the nearby neurons regardless of the scale.}, representing how likely a neuron i  inhibits a neuron j. As such, each active neuron inhibits its weaker neighbours, introducing a locality in the network inspired by biological neurons. While the notion of neighbouring neurons is not well established in a fully connected network, our aim is to allow few  neurons to be active and not only one, thus those few activations don't have to be small to compensate for the penalty. $\sigma^2$ is a hyper parameter representing the scale at which neurons can affect each other. Our regularizer inhibits locally the  active neurons leading to a sparse coding through local neural inhibition, hence the name of our regularizer Sparse coding through Local Neural Inhibiation, {\tt SLNI} for short.  
\\
This is applied for each task in the learning sequence. In the case of  tasks with completely different input patterns, the active neurons of the previous tasks will not be activated given the new tasks input patterns. However, when the new tasks are of similar
or shared patterns, neurons used for previous tasks will be active and our penalty would discourage other neurons from being active and encourage the new task to adapt the already active neurons instead. This would interfere with the previous tasks and could increase forgetting which is exactly what we want to overcome. To avoid such interference, we  set a weight factor according to the importance of the neurons with respect to the previous tasks. To estimate the importance of the neurons 
for a given task, we utilize a similar \marcus{same or similar. if similar, we should state the difference} criteria to that when estimating the parameters importance in \cite{aljundi2017memory} \marcus{what is specific to \cite{aljundi2017memory}? what changes when using it with \cite{kirkpatrick2016overcoming}. It might be better to have the method section more independent of \cite{aljundi2017memory}.}\rahaf{it is either we use the gradient w.r.t the loss or the output layer} i.e. the sensitivity of the learned function to their changes  approximated by the gradients of the learned function w.r.t. the parameters at the end of a training phase. Here, we consider our variables to be the neurons output and use the gradient of the output layer evaluated at each data point. To get an importance measure, we then accumulate the magnitude of the gradients over the given data points %
to obtain importance weight $\alpha_{i}$ for a neuron $n_{i}$: 
\begin{equation}\label{eq:2}
\alpha_{i} =\frac{1}{M}\sum_{m=1}^M  \mid\mid g_{i}(x_m) \mid\mid \quad,\quad g_{i}(x_m)=\frac{\partial (F(x_m))}{\partial n^{m}_{i}}
\end{equation}
Where $n^{m}_{i}$ is the output of the neuron $n_i$ for a given input example $x_m$.\\
Then, we weight our {\tt SNI} regularizer as follows:
\marcus{do you have any ablations for adding $e^{-(\alpha_{i}+\alpha_{j})}$}
\marcus{I would only call the final version $R_{SNI}$ and not already the one in Eq \ref{eq:appraoch:regularizer:first} [Edited]}
\rahaf{I am not sure I understand your comment}
\begin{equation} 
\label{eq:appraoch:regularizer:final}
R_{\textrm{SNI}}(H_l)=\frac{1}{M}   \sum_{i,j}\frac{P(x_{ij})}{P(0)} e^{-(\alpha_{i}+\alpha_{j})}\sum_m h_i^mh_j^m ,  \quad i\neq j
\end{equation}
which can be read as: if  an important neuron for a previous task is active given  an input pattern from the current task, it will not suppress the other neurons from being active neither be affected by other active neurons.
Adding all the terms will result in the following objective for training a later task in a sequence:
\begin{equation}
\label{eq:appraoch:loss:final}
T_{t}: \quad \min_{\theta} \frac{1}{M} \sum_{m=1}^{M} l(y_m,f(x_m,\theta))+\lambda_{\textrm{SNI}} \sum_{l} R_{\textrm{SNI}}(H_l) +\lambda_{\Omega}\sum_{k} \Omega_{k}(\theta_{k}-\theta^*_{k})^2
\end{equation} 
 $\lambda_{\textrm{SNI}}$ and  $\lambda_{\Omega}$ are trade-off parameters that control the contribution of each term.
When training the first task, ${\alpha_i}=0$ and  $\Omega_{ki}=0$, which means that for the first task Eq \ref{eq:appraoch:regularizer:final} simplifies to Eq \ref{eq:appraoch:regularizer:first}.


==> intro_old.tex <==
%\marcus{[Marcus: is this really the case? One could e.g. store the support vectors of previous tasks? or store some previous outputs/Knowledge Distillation]}
%\marcus{[Marcus: the first sentence has too many key words]}
Sequential learning, also referred to as continual learning or lifelong learning, studies the problem of learning a %open 
sequence of tasks without access to the training data of previous tasks and at the same time avoiding catastrophic interference with 
the previously learned tasks. Catastrophic interference or catastrophic forgetting is the severe forgetting of previous tasks \citep{french1999catastrophic}. While avoiding such catastrophic interference is not possible using learning methods like SVM \citep{goodfellow2013empirical}, it is more plausible in neural networks. 
    Since the early development of neural networks, researchers have faced the catastrophic forgetting problem and developed several strategies to mitigate the forgetting under the condition of not storing the previous tasks training data~\citep{kruschke1992alcove,ans1997avoiding,robins1995catastrophic}. Recently, and after the return  of neural networks, the catastrophic forgetting problem and the sequential learning paradigm  received increased attention. Similar or new approaches have been proposed to maintain the previous tasks performance and prevent forgetting. While some methods proceed by storing %\marcusadd{or some previous task data \citep{lopez2017gradient} or} 
     previous tasks models \citep{aljundi2016expert,rusu2016progressive,lee2017overcoming}  and at test time, selecting one model or merging the models, here, we are interested in the challenging situation of learning a sequence of tasks {\em using a fixed  model capacity}. % and no access to any task previous data}. 
%\item importance of learning sequence of tasks using one model


This has the advantage of not increasing the memory demand nor the processing time while allowing knowledge sharing and transfer between tasks resulting in scalable lifelong learning methods.  Under this constraint, proposed methods either follow a pseudo rehearsal approach \citep{li2016learning,rannen2017encoder} or rely on penalizing changes to the parameters that are important for the previous tasks~\citep{kirkpatrick2016overcoming,zenke2017improved,aljundi2017memory,chaudhry2018riemannian,liu2018rotate}. This latter line avoids issues related to the distribution shift between the different tasks data but highly %correlates with
depends on the percentage of parameters used to solve the previous tasks and hence the capacity that is left  for the new tasks. % consider introducing here the relation between important weigths and free model capacity, now lines 80-84.
This %can be seen as the 
results in a performance on the newly learned tasks that is considerably lower than when learning these tasks alone.  At the same time, when learning a similar set of tasks jointly, %would result on 
it is often possible to obtain
good performance for all the tasks~\citep{aljundi2016expert}. This indicates that the network actually has enough capacity to  host all the tasks. In fact, it is well known that neural networks represent complex functions and the learning procedure converges into a local minimum. To achieve a good performance on the task being learned, different %approximations 
solutions can be found which differ in their complexity and hence  the amount of parameters and corresponding neurons they utilize. While most of the regularization techniques aim at reducing overfitting, little attention has been dedicated to the sparsity of the learned solution as a goal per se. 
\marcus{I think the first two paragraphs are two general and not enough to the point of the problem we are looking at. [In other words the first to paragraphs should be more "selfless";)]}

%If we consider 
The mammalian brain is composed of billions of neurons but, at the same time, information is represented by only a few active neurons resulting in a sparsity of 90-95\%~\citep{lennie2003cost}.  
%Through lateral inhibition of excited neurons to their weaker neighbors,  a powerful decorrelated and compact representation is obtained with minimum interference between different patterns~\citep{yu2014sparse}. 
In neural biology, \emph{lateral inhibition} describes the ability of an activated neuron to reduce the activity of its weaker neighbors. This creates a powerful decorrelated and compact representation with minimum interference between different input patterns~\citep{yu2014sparse}. 
On the  contrary, neural networks learn dense representations that are highly entangled and sensitive to changes in the input~\citep{bengio2009learning}. We argue that a sparse and decorrelated
representation would be less sensitive to new and different patterns (such as data from new tasks), meanwhile allowing the training procedure of the new tasks to re-use those possibly free neurons with less interference with the previous tasks.
% consider introducing here a definition for "sparsity".
\marcus{maybe this a nice first paragraph for the paper... We already said about sequential learning in the abstract}

In general, sparsity in neural networks can be thought of either in terms of the network parameters or in terms of the representation (i.e., the activations). Differently from most of the compression based approaches~\citep{liu2015sparse,aghasi2017net,louizos2017bayesian}, we argue that, in a sequential learning scenario,  achieving sparsity in the network parameters is less significant  than sparsity in the neural activations. Indeed, when the effective  parameters are spread among the different neurons,  changing the ineffective ones would change the function of their corresponding neurons and hence interfere with previous tasks. 


To this end, we study the effect of regularization techniques and activation functions on the performance of sequential learning. %that aim at learning sparse or decorrelated representations.
Based on finding that we need sparse activations, as core contribution of this work, we propose a new regularizer that exhibits a behavior similar to the lateral inhibition in  biological neurons. %  without the spatial criteria.
 It results in a sparse and decorrelated representation of different input patterns. When accompanied with a state-of-the-art important parameters preservation method, it leads to an improved performance in all the tasks, specially the lastly learned ones, compared to the standard sequential learning procedure. %meaning finetuning or the vanilla application of EWC or MAS? \\

% \item running out of capacity and importance of sparsity\\
% This phenomena seems expectable in the case of a fixed capacity model. However,in this paper we study the possibility of guiding the currently  learned task towards using fewest amount of neurons and its influence on the performance of the later tasks. Our hypothesis is based on the fact that neural netowrks represent complex functions and the learning procedure converges into a local minima. Hence, to achieve a good performance on the task being learned, different approximations can be found in which they differ by the amount of parameters and corresponding neurons they utilize. While most of the regularization methods aim at reducing overfitting, little attention have been dedicated to the sparsity of the learned solution. On the other hand, our brain are highly sparse where only 90-95\% of the neurons are active at a given time (add ref). We argue in this paper that achieving higher rates of sparsity in the neural network not only leads to a less computations at a time but a far more less overlapped representation between the different tasks. This would minimize the interference between the different tasks and increase the performance of each individual task.
In the following, we first discuss the different approaches for lifelong learning and then discuss different regularization criteria that from a lifelong learning perspective  (Section~\ref{sec:related}). We proceed by proposing our approach that promotes sparsity and decorrelation through neural inhibition (Section~\ref{sec:method}). Section~\ref{sec:experiments} describes our experimental evaluation, while Section~\ref{sec:conclusion} concludes the paper.


==> old_approach.tex <==
\section{OLD PART: Regularization in Sequential Learning}\label{sec:approaches}
We study possible regularization techniques that could lead to less interference between the different tasks in a sequential learning scenario either by enforcing sparsity or decorrelation. Additionally, we examine the use of  activation functions that are inspired by lateral inhibition in biological neurons that could be advantageous in sequential learning. \\
\textbf{Representation Based methods:} \\
-~{\tt L1-Rep}: since using $L_0$ norm is an NP hard problem, the most natural alternative to learn sparse representation  is an $L_1$ norm on the neurons activations. This leads to an equal penalty on all the active neurons for a given example. It has been  suggested by~\cite{pmlr-v15-glorot11a} to be combined with the rectifier activation function (ReLU)~\citep{pmlr-v15-glorot11a} to control the unbounded activations and to increase the sparsity.\\
- {\tt Decov}~\citep{cogswell2015reducing}   aims at reducing overfitting by decorrelating  neuron activations. To do so, it minimizes the Frobenius norm of the  covariance matrix computed on the activations of the current  batch after subtracting the diagonal to avoid  penalizing independent  neuron activations. \\
- {\tt Maxout} network~\citep{goodfellow2013maxout} utilizes the maxout activation function. For each group of neurons, based on a fixed window size, only the maximum activation is forwarded to the next layer. The activation function guarantees a minimum sparsity rate defined by the window size.  \\
- {\tt LWTA}~\citep{NIPS2013_5059}: similar idea to the Maxout network with the difference that the non maximum activation are set to zero while maintaining their connections. In contrast to Maxout, LWTA keeps the connections of the inactive neurons which can be occupied later once they are activated without changing the previously active neuron connections.\\
\textbf{Parameters based regularizers:} \\
-{\tt OrthReg}~\citep{rodriguez2016regularizing}: Regularizing CNNs with locally constrained decorrelations. It aims at decorrelating the feature detectors  by minimizing the cosine of the angle between the weight vectors resulting eventually in orthogonal weight vectors.\\
-{\tt L2-WD}: Weight decay with $L_2$ norm ~\citep{krogh1992simple} controls the complexity of the learned function by minimizing the magnitude of the weights.\\
-{\tt L1-Param}:  $L_1$ penalty on the parameters  to encourage a solution with sparse parameters.

Dropout is not considered as its role contradicts our goal. While dropout can improve each task performance and reduce overfitting, it acts as a model averaging technique.   By randomly masking neurons, dropout forces the different neurons to work independently but as a result encourages redundant representation. As shown by~\citep{goodfellow2013empirical} the best network size for classifying  MNIST digits was when using dropout about $50\%$ more than without it. Dropout steers the learning of a task to towards occupying a good portion of the network capacity if not all of it which contradicts with the sequential learning needs.

\myparagraph{Parameter sparsity vs. representation sparsity.}
As we explained in the introduction%~\ref{sec:intro}
, from a sequential learning point of view, sparsity in the representation is more advantageous than sparsity in the  network parameters.
If we encourage sparsity in the parameters independently from their corresponding neurons, the learning of a task could result in few non zero parameters spread across the different neurons. When a new task uses the free parameters by changing those with zero values, it would interfere with the previously learned representation and result in a deterioration of the previous task performance. On the other hand, when few neurons are active and hence used by the first task, other neurons can be used by later tasks without negative impact on the learned representation as shown in Figure~\ref{fig:param_vs_rep}.
\begin{figure*}[t]
\centering
\vspace*{-0.2cm} 
\includegraphics[width=0.95\textwidth]{images/PMvsRP.pdf} 
  \caption{The difference between parameter sparsity (a) and representation sparsity (b) in a simple case of two tasks. Learning the first task utilized parts indicated in red. The second task has different input pattern and re-used parts shown in green. Orange indicates shared neurons. In (a), when an example from the first task  is encountered again, the activations of the first layer will not be affected by the changes, however, the second layer activations will be changed affecting the output of the second task. Such interference is avoided when achieving sparsity on the representation (b). }  
  \label{fig:param_vs_rep}
  \vspace*{-0.8cm} 
\end{figure*}


\section{Sparse coding through Neural Inhibition (\textbf{SNI})}
\label{sec:method}

\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}

The previously  presented regularizers either encourage sparsity by penalizing all the active neurons or encourage neural decorrelation but lack sparsity. While the idea of lateral inhibition depicted in Maxout~\citep{goodfellow2013maxout} and LWTA~\citep{NIPS2013_5059} is interesting and powerful~\citep{maass2000computational}\marcus{it is a bit surprising that a citation from 2000 can show that something is interesting and powerful published in 2013... maybe reformulate?}, it remains restricted to a fixed window size.
Our objective is to achieve the least number of active neurons while maintaining a powerful representation. In other words, we want the neurons with high activations to inhibit the other neurons with the goal of achieving sparse coding through neural inhibition in a similar spirit 
to the process observed in biological neurons. To proceed, we consider a hidden layer $l$ with the activations $H_l=\{h^m_{i}\}$ given an input example $x_m$ where $i \in {1,..,N}$ with $N$ the  number of neurons in the hidden layer and $m \in {1,..,M}$ with $M$ the number of examples. When a neuron is active, we want to have a minimal number of other active neurons  at the same time. In a sense, we want to minimize the correlated activations, %in example bases \marcus{[not necessary clear what example bases is]}. 
%this boils down to 
which can be achieved by minimizing the cross covariance   $C_{i,j}$ between individual neurons activations $\{h_i,h_j\}$ 
\begin{equation}
C_{ij}=\frac{1}{M}  \sum_m (h_i^m -\mu_i )(h_j^m -\mu_j)
\end{equation}
with $\mu_{i}$/$\mu_{j}$ the mean activation value of neuron $i$/$j$. %Marcus: don't use k as it is used later
% To do so, we propose to minimize  the $L_1$ norm of the neurons' cross covariance 
% \begin{equation}
% L=\|C\| -\|diag(C)\|=\frac{1}{N} \sum_i\sum_{j\neq i}  | h_i^m -\mu_i )(h_j^m -\mu_j|
% \end{equation}
In the case of a ReLU activation function, which is used in most of the modern architectures, a neuron is active  if its output is larger than zero and zero otherwise. We want to have a decorrelated representation that is highly sparse in which the neurons activations are zero most of the time unless an important pattern has been detected. Hence, by assuming that the mean of the activations is close to zero,
%
% Thus, we consider having a mean close to zero  to discourage the neurons' activations from frequently having nonzero values.  in 
%\begin{equation}
$ \mu_i \simeq 0 \, \forall i \in {1,..,N}$
%\end{equation}
we propose to minimize the following:
\begin{equation}
R_{\textrm{SNI}}(H_l)=\frac{1}{M}  \sum_{i,j}\sum_m w_{ij} h_i^mh_j^m  ,  \quad i\neq j
\end{equation}
 $w_{ij} $ is a weighting factor -- let's ignore it for the moment. To understand the  function of this regularizer, let's  compute its  derivative with respect to a particular activation $h_i^m$  
\begin{equation}
\label{eq:appraoch:regularizer:first}
\frac {\partial R_{\textrm{SNI}}(H_l)}{\partial h_i^m}=\frac{1}{M}   \sum_{j\neq i} w_{ij} h_j^m
\end{equation}
We can see that each active neuron receives a penalty from every other active neuron that corresponds to that other neuron's activation magnitude. In other  words, if a neuron fires, with a high activation value, for a given example, it will suppress firing other neurons for that same example, hence the name of our regularizer Sparse coding through Neural Inhibition, {\tt SNI} for short.  Ultimately, we will have a minimal number of active neurons resulting in a sparse neural coding. Note that this differs from an $L_1$ norm to the neurons activations that penalizes equally all the active neurons. 
%While we encourage sparsity given each  example independently, it is highly probable that sparsity over the different examples will be achieved at the end of the learning. When a neuron is active, it means that it is detecting a pattern in this example and hence it will be active whenever a similar pattern is seen in other examples.
When learning the first task, our regularizer is combined with the corresponding task loss 
\begin{equation}
\label{eq:appraoch:loss:first}
T_1:\quad \min_{\theta} \frac{1}{M} \sum_{m=1}^{M}  l(y_m,f(x_m,\theta))+\lambda_{\textrm{SNI}} \sum_{l} R_{\textrm{SNI}}(H_l)
\end{equation}
 the input $x_m$ and the desired output $y_m$ of the network; and $\lambda_{\textrm{SNI}}$ a trade-off parameter.



To achieve sequential learning, when moving to a second task and to prevent the forgetting of the previous task knowledge, we employ  state-of-the-art methods~\citep{aljundi2017memory,kirkpatrick2016overcoming} that estimate importance weight $\Omega$ on the network parameters for a given task.  While learning a new task, the changes on the important parameters are discouraged using $L_2$ penalty:
%\begin{equation} 
$\min_{\theta} \sum_{i,j} \Omega_{ij}(\theta_{ij}-\theta^*_{ij})^2$, where 
%\end{equation}
$\theta^*_{ij}$ are the optimal parameters that are learned so far, i.e. before the current task.

Now back to the weight factor $w_{ij}$ introduced earlier. If we set it naively to 1, then our regularizer will affect similarly all the activations.  In the case of  tasks with completely different input patterns, the active neurons of the previous tasks will not be activated given the new tasks input patterns. However, when the new tasks are of similar or shared patterns, neurons used for previous tasks will be active and setting $w_{ij}$ to $1$ would discourage other neurons from being active and encourage the new task to adapt the already active neurons instead. This would interfere with the previous tasks and could increase forgetting which is exactly what we want to overcome. To avoid such interference, we  set the weight factor according the importance of neurons with respect to the previous tasks. To this end, we consider an importance estimate of each neuron as the sum of the parameters importance that are connected, as input, to that neuron.
\begin{equation}
\alpha_{i}=\frac{1}{N_{l-1}}\sum_{k=1}^{N_{l-1}}\Omega_{ki}
\end{equation}
where $\Omega$ is the parameters importance matrix of layer $l$, 
computed using MAS~\citep{aljundi2017memory} or EWC~\citep{kirkpatrick2016overcoming}; $N_{l-1}$ is the number of neurons in layer ${l-1}$.  Then, we weight our {\tt SNI} regularizer as follows
\begin{equation}
\label{eq:appraoch:regularizer:final}
R_{\textrm{SNI}}(H_l)=\frac{1}{M} \sum_{i,j}\sum_m e^{-(\alpha_{i}+\alpha_{j})} h_i^mh_j^m ,  \quad i\neq j
\end{equation}
which can be read as: if  an important neuron for a previous task is active given  an input pattern from the current task, it will not suppress the other neurons from being active neither be affected by other active neurons.
Adding all the terms will result in the following objective for training a later task in a sequence:
\begin{equation}
\label{eq:appraoch:loss:final}
T_{t}: \quad \min_{\theta} \frac{1}{M} \sum_{m=1}^{M} l(y_m,f(x_m,\theta))+\lambda_{\textrm{SNI}} \sum_{l} R_{\textrm{SNI}}(H_l) +\lambda_{\Omega}\sum_{i,j} \Omega_{ij}(\theta_{ij}-\theta^*_{ij})^2
\end{equation} 
 $\lambda_{\textrm{SNI}}$ and  $\lambda_{\Omega}$ are trade-off parameters that control the contribution of each term.
When training the first task, $\Omega_{ki}=0$, which means that for the first task Eq \ref{eq:appraoch:regularizer:final} simplifies to Eq \ref{eq:appraoch:regularizer:first} and Eq \ref{eq:appraoch:loss:final} to \ref{eq:appraoch:loss:first}. %with $w_{ij}=1$. \marcus{["with $w_{ij}=1$" could be removed, $w_{ij}=1$ if $\Omega_{ki}=0$, or?]} \tinne{I guess we can leave out this last sentence}

